ONE-PEACE: Exploring One General Representation Model Toward Unlimited Modalities

In this work, we explore a scalable way for building a general representation model toward unlimited modalities. We release ONE-PEACE, a highly extensible model with 4B parameters that can seamlessly align and integrate representations across vision, audio, and language modalities. The architecture of ONE-PEACE comprises modality adapters, shared self-attention layers, and modality FFNs. This design allows for the easy extension of new modalities by adding adapters and FFNs, while also enabling multi-modal fusion through self-attention layers. To pretrain ONE-PEACE, we develop two modality-agnostic pretraining tasks, cross-modal aligning contrast and intra-modal denoising contrast, which align the semantic space of different modalities and capture fine-grained details within modalities concurrently. With the scaling-friendly architecture and pretraining tasks, ONE-PEACE has the potential to expand to unlimited modalities. Without using any vision or language pretrained model for initialization, ONE-PEACE achieves leading results on a wide range of uni-modal and multi-modal tasks, including image classification (ImageNet), semantic segmentation (ADE20K), audio-text retrieval (AudioCaps, Clotho), audio classification (ESC-50, FSD50K, VGGSound), audio question answering (AVQA), image-text retrieval (MSCOCO, Flickr30K), and visual grounding (RefCOCO/+/g). Code is available at https://github.com/OFA-Sys/ONE-PEACE.

==> content/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% Multi-modality signals are entangled in the real world.

% With the rapid development of deep learning, it has become possible to build such a general AI system. 
% First, the recent progress of Transformer shows it has the potential to become a general model applicable to multiple modalities. Second, pretraining techniques have achieved remarkable success across different domains, enabling models to have strong generalization capabilities and efficiently transfer to various tasks.

% We think that there are several reasons for this:
% Firstly, models used in different modalities differ greatly. Although the popularity of Transformers in recent years has made models from different fields gradually converge, a single Transformer structure is still difficult to accurately represent the features of each modality.
% Secondly, due to the different characteristics of different modalities, it is difficult to use a unified pre-training task to train the model. For example, text is discrete data, while images and speech are continuous data. A common solution is to cluster or introduce additional models to discretize continuous data, and then train the model through masked prediction tasks. However, these discretization operations also increase the difficulty of training.
% Finally, multi-modal models need to pay attention to both intra-modal and cross-modal tasks, which means that the model needs to learn the information within each modality while also focusing on alignment between modalities. This inevitably requires the introduction of multi-task training methods, which often have conflicts.
% This article focuses on building a universal representation model, hoping to simultaneously model the data of images, text, and audio through a unified architecture and pre-training tasks.
% We have built a universal representation model called ONE-PEACE, whose model architecture is based on a Transformer Model. It consists of multiple modality-specific adapters and a modality fusion encoder, which includes multiple modality-specific FFNs and modality-shared self-attention layers.
% To efficiently extract information within each modality and align different modalities' semantic spaces, we have designed two contrastive-style pre-training tasks: cross-modal contrastive learning and masked intra-modal contrastive learning. These two tasks can work well together, allowing the model to achieve superior finetuning performance in downstream tasks while maintaining good zero-shot cross-modal retrieval capabilities.

% Building a general AI system is a fascinating and challenging goal. Such a system should not only perform well in individual modalities but also be able to handle multiple modalities simultaneously. It requires the system to accurately comprehend the semantics of various modalities and align the semantic space of different modalities.

% With the rapid development of deep learning, building a general AI system is become possible. Firstly, 

% In recent years, large-scale pretrained models have achieved remarkable success across different domains, including natural language processing, computer vision, speech processing, etc.
% Some researchers also explore vision-language pretraining and audio-language pretraining, and have achieved promising results in downstream tasks. However, models that can simultaneously model vision, audio, and language are still relatively rare. 

% There are several reasons for this:
% Firstly, models used in different modalities differ greatly. Although the popularity of Transformers in recent years has made models from different fields gradually converge, a single Transformer structure is still difficult to accurately represent the features of each modality.
% Secondly, due to the different characteristics of different modalities, it is difficult to use a unified pre-training task to train the model. For example, text is discrete data, while images and speech are continuous data. A common solution is to cluster or introduce additional models to discretize continuous data, and then train the model through masked prediction tasks. However, these discretization operations also increase the difficulty of training.
% Finally, multi-modal models need to pay attention to both intra-modal and cross-modal tasks, which means that the model needs to learn the information within each modality while also focusing on alignment between modalities. This inevitably requires the introduction of multi-task training methods, which often have conflicts.

% In this paper, we propose \onepeace. a general representation model that can handle language, vision, audio, and multimodal tasks. 
% The model architecture of \onepeace consists of multiple modality-specific adapters and a modality fusion encoder.
% To efficiently extract information within each modality and align different modalities' semantic spaces, we have designed two contrastive-style pre-training tasks: cross-modal contrastive learning and masked intra-modal contrastive learning. These two tasks can work well together, allowing the model to achieve superior finetuning performance in downstream tasks while maintaining good zero-shot cross-modal retrieval capabilities.


Building a general AI system is a fascinating and challenging goal. Such a system should not only perform well in individual modalities but also be able to handle multiple modalities simultaneously. It requires the system to accurately understand the semantics of various modalities and align the semantic spaces of different modalities. With the rapid development of deep learning, building a general AI system is gradually becoming possible.



% In the past years, model architectures vary greatly in different domains.
% For example, models in natural language processing (NLP) were mainly based on recurrent neural networks (RNNs), while models in computer vision (CV) were mainly based on convolutional neural networks (CNNs).
% With the rise of Transformers~\cite{transformer,vit}, model architectures across different domains gradually begin to converge. It is possible to process all modalities through a unified Transformer model.
% For the training method, the “pretrain-finetune” paradigm has achieved remarkable success across various domains, including NLP, CV, speech processing, etc.
% To enhance the ability of pretrained models, various pretraining tasks have been proposed. Masked language modeling is a classic pretraining task that has been proven effective in multiple domains. 
% It learns data by reconstructing randomly masked units and can help models achieve excellent finetuning performance in downstream tasks.
% Cross-modal Contrastive learning is one of the representatives of cross-modal pretraining tasks, which can effectively align the semantic space of different modalities and enable the model to have strong cross-modal retrieval ability.

Firstly, model structures across different domains gradually begin to converge. In the past years, the architectures varied greatly in different domains, such as recurrent neural networks (RNNs)~\cite{rnn} and convolutional neural networks (CNNs)~\cite{mnist}.  With the development of Transformer~\cite{transformer,vit}, researchers have successfully applied Transformer to various domains.  It has now become possible to process all modalities through a unified Transformer model.
Secondly, the “pre-train then finetune” paradigm has achieved remarkable success in natural language processing~\cite{bert,gpt,gpt3,electra,roberta,deberta,xlnet,bart,T5}, computer vision~\cite{beit,mae,ibot,moco,mocov2,mocov3,simclr}, speech processing~\cite{wav2vec,wav2vec2,wavlm,hubert}, etc. To enhance the ability of pre-trained models, various pre-training tasks have been proposed. Masked prediction is a pre-training task that has proven effective in multiple domains, which learns data by reconstructing randomly masked units and can help models achieve excellent finetuning performance in downstream tasks. Cross-modal contrastive learning is one of the representatives of cross-modal pre-training tasks, which can effectively align the semantic space of different modalities and enable the model to have strong cross-modal retrieval ability.

With the help of a unified model structure and efficient pre-training tasks, recent works have achieved promising results in vision-language learning~\cite{ofa,flamingo,coca,beit3,blip,pali} and audio-language learning~\cite{audioclip,wav2clip,clap,speecht5,speechlm}. However, there is still a lack of research on developing general models that can be applied to visual, audio, and language tasks. This paper focuses on building a general representation model. We advocate that a general representation model should meet the following conditions:
1). The model architecture needs to be sufficiently flexible. Ideally, the model should incorporate modality-specific components to capture modality-specific information, as well as modality-interaction components to enable cross-modal interaction.
2). The pre-training tasks should be general and simple enough to apply to different modalities. 
3). The pre-training tasks should not only focus on extracting information within each modality but also ensure alignment across modalities so that the model can achieve good performance in both single-modality tasks and multi-modality tasks.

% There are several reasons for this:
% Firstly, although the popularity of Transformers in recent years has made models from different fields gradually converge, a single Transformer structure is still difficult to accurately extract the features of each modality.
% Secondly, due to the different characteristics of different modalities, it is difficult to design a unified pretraining task to train the model. For example, text is discrete data, while images and speech are continuous data. A common solution is to cluster or introduce additional models to discretize continuous data, and then train the model through masked prediction tasks. However, these discretization operations also increase the difficulty of training.
% Finally, multi-modal models need to pay attention to both intra-modal and cross-modal tasks, which means that the model needs to learn the information within each modality while also focusing on alignment between modalities. This inevitably requires the introduction of multi-task training methods, which often have conflicts.

In this paper, we propose \onepeace. a general representation model that can handle language, vision, audio, and multimodal tasks. 
The model architecture of \onepeace consists of multiple modality-specific adapters and a modality fusion encoder. The modality fusion encoder is based on the Transformer architecture, we set up a shared self-attention layer and multiple modality-specific Feed Forward Networks (FFNs) in each Transformer block.
With such a flexible model structure, introducing new modalities is a straightforward process that only requires the addition of modality-specific parts.
To efficiently extract information within each modality and align the semantic spaces of different modalities, we design two contrastive-style pretraining tasks: cross-modal contrastive learning and masked intra-modal contrastive learning. These two tasks can work well together, allowing the model to achieve superior finetuning performance in downstream tasks while maintaining good zero-shot cross-modal retrieval capability.

We conduct comprehensive experiments to demonstrate the effectiveness of \onepeace. Experimental results show that \onepeace achieves state-of-the-art results on cross-modal and single-modal tasks, including visual grounding, image-text retrieval, and object segmentation.

% Our main contributions are summarized as follows:
% \begin{itemize}
%     \item We propose a general representation model \onepeace that can handle language, vision, audio, and multimodal tasks. The model architecture of \onepeace consists of modality-specific modules and modality-sharing modules, which have the potential to expand to infinity modalities.
%     \item We combine both cross-modal contrastive learning and masked intra-modal contrastive learning to pretrain \onepeace.
%     These tasks are well-compatible, allowing the model to achieve superior finetuning performance in downstream tasks while maintaining good zero-shot cross-modal retrieval capability.
%     \item We conduct comprehensive experiments to demonstrate the effectiveness of \onepeace. Experimental results show that \onepeace achieves state-of-the-art results on cross-modal and single-modal tasks, including visual grounding, image-text retrieval, and object segmentation.
% \end{itemize}







==> content/3_method.tex <==
\section{Method}
\label{sec:method}

\begin{figure*}[t]
\vskip 0.2in
    \centering
    \includegraphics[width=0.7\linewidth]{pic/model.pdf}
    \caption{\textbf{The model achitecture of \onepeace}. The model is composed of multiple components that are specific to each modality (e.g., vision adapter) as well as components that are shared across modalities (e.g., self-attention layer). Different combinations of modules can be used to perform various tasks. For instance, the combination of vision adapter, self-attention layers, and vision FFNs can be utilized for vision tasks.}
    \label{fig:model}
\end{figure*}

% 在这里直接介绍整个framework
% \onepeace~consist of multiple modality-specific adapters and a modality fusion encoder.
% We pretrain \onepeace~through both inter-modal contrastive learning and masked intra-modal contrastive learning. 
% The overall framework is illustrated in Figure xxx.

% % 介绍这个章节的内容
% In this section, we first describe the overall model architecture of \onepeace. Next, we describe the pretraining tasks: Vision(Audio)-Language Contrastive Learning and Maksed Contrastive Learning. Finally, we introduce the pretraining details of \onepeace, including datasets and pretrainng setup.

% % 整体介绍模型架构
% The overall model architecture consists of multiple modality-specific adapters and a Multiway Transformer~\cite{beit3}. 

\subsection{Architecture}
In this section, we introduce the model architecture of \onepeace, which consist of multiple modality-specific adapters and a modality fusion encoder.
The overall architecture is shown in Figure~\ref{fig:model}.

% We pretrain \onepeace~through both inter-modal contrastive learning and masked intra-modal contrastive learning. 
% The overall framework is illustrated in Figure xxx.

\subsubsection{Modality-Specific Adapters}
%Vision, audio, and text modalities have different characteristics. 
%In order to process the inputs of these modalities into appropriate representations, we introduce three modality-specific adapters: vision adapter, audio adapter, and language adapter. 
% Distinct characteristics are exhibited by vision, audio, and language. To facilitate the processing of modality-specific inputs and transform them into representations, we propose three modality-specific adapters: vision adapter (V-Adapter), audio adapter (A-Adapter), and language adapter (L-Adapter).
% These adapters will process the inputs of the corresponding modality and transform them into a series of embedding sequence.

Different modalities exhibit distinct characteristics.
To facilitate the processing of modality-specific inputs, we design modality-specific adapters to process data from each modality individually.
Note that these adapters do not interfere with each other and are solely responsible for converting the raw input into vectors.
This affords us the flexibility to choose the appropriate networks for the adapters, which can be Transformers~\cite{transformer,vit,swin}, CNNs~\cite{cnn,resnet}, RNNs~\cite{rnn,gru,lstm}, etc.
In this paper, we design three modality-specific adapters for \onepeace, including vision adapter, audio adapter, and language adapter.

\paragraph{Vision Adapter}
Given an image $I$, we use a hierarchical MLP (hMLP) stem~\cite{Touvron2022ThreeTE} to patchify the image by gradually increasing the patch size to $16 \times 16$. Note that there is no interaction between different patches. Then the image patches are flattened to a sequence and prepended with a vision class embedding. By adding the absolute positional embeddings into the image embeddings, we derive the image input representation $E^V=\langle \bm{e}^V_{cls}, \bm{e}^V_{1}, \bm{e}^V_{2}, ..., \bm{e}^V_{M} \rangle$, where $M$ denotes the total number of image patches.
%The image patches are then flattened to an image embedding sequence with a prepend vision class embedding, by adding the absolute positional embeddings to the image embeddings, we finally obtain the image input representation $E^V=\langle e^V_{cls}, e^V_{1}, e^V_{2}, ..., e^V_{M} \rangle$, where $M$ is the number of image patches.

\paragraph{Audio Adapter}
Given an audio $A$, we set the sample rate to 16kHz and normalized the raw waveform input to zero mean and unit variance. Then the normalized waveform is processed by a convolutional feature extractor~\cite{wav2vec2} to get the audio embeddings. Instead of using the absolute positional embeddings, we use a convolution layer to extract relative position information and add it to the audio embeddings~\cite{Mohamed2019TransformersWC}. With a prepended audio class embedding, we finally obtain the audio input representation $E^A=\langle \bm{e}^A_{cls}, \bm{e}^A_{1}, \bm{e}^A_{2}, ..., \bm{e}^A_{N} \rangle$, where $N$ denotes the length of the audio.
 
\paragraph{Language Adapter}
Given a text $T$, we first apply byte-pair encoding (BPE) \cite{bpe} to transform it to a subword sequence. Two special tokens $\left[{\rm CLS}\right]$ and $\left[{\rm EOS}\right]$ are inserted at the beginning and end of the sentence to indicate its start and end. Then an embedding layer is used to embed the subword sequence to the text embeddings. After summing the text embeddings and absolute positional embeddings, we obtain the text input representation $E^L=\langle \bm{e}^L_{cls}, \bm{e}^L_{1}, \bm{e}^L_{2}, ..., \bm{e}^L_{K}, \bm{e}^L_{eos} \rangle$, where $K$ denotes the text sequence length.

\subsubsection{Modality Fusion Encoder}
Following previous works~\cite{simvlm,ofa,coca,beit3}, the modality fusion encoder is based on the Transformer architecture~\cite{transformer}. 
To make it more suitable for different modalities, we make the following improvements:

\paragraph{Modality-Specific FFNs} 
To facilitate the interaction between different modalities while capturing modality-specific information, we set up a shared self-attention layer and three modality-specific feed-forward networks (FFNs) in each Transformer block.
The shared self-attention layer enables the interaction between different modalities through the attention mechanism.
The three modality-specific FFNs include vision FFN (V-FFN), audio FFN (A-FFN), and language FFN (L-FFN), which can further extract information within their respective modalities after modality interaction.
% This "shared-separate" structure is largely inspired by~\cite{vlmo,beit3}, 
We find it can achieve better results compared with the vanilla Transformer architecture. 
Furthermore, this structure can be disassembled into different branches to handle the tasks of various modalities.
For example, the vision adapter, self-attention layer, and vision FFNs can be combined into the vision branch (V-Branch) to process visual tasks.
Similarly, we named other branches as A-Branch, L-Branch, VA Branch, VL-Branch, AL-Branch, and VAL-Branch.
% Furthermore, this structure can be disassembled into the following branches to handle the tasks of various modalities:

% \begin{itemize}
% \item \textbf{Vision Branch} (V-Branch) contains the vision adapter, shared self-attention layers, and vision FFN. This branch is used to process vision tasks.
% \item \textbf{Audio Branch} (A-Branch) contains the audio adapter, shared self-attention layers, and audio FFN. This branch is used to process audio tasks.
% \item \textbf{Language Branch} (L-Branch) contains the language adapter, shared self-attention layers, and language FFN. This branch is used to process language tasks.
% \item \textbf{Vision-Language Branch} (VL-Branch) contains the vision adapter, language adapter, shared self-attention layers, vision FFN, and language FFN. This branch is used to process vision-language tasks.
% \item \textbf{Audio-Language Branch} (AL-Branch) contains the audio adapter, language adapter, shared self-attention layers, audio FFN, and language FFN. This branch is used to process audio-language tasks.
% \item \textbf{Vision-Audio-Language Branch} (VAL-Branch) contains all the adapters, self-attention layers, and FFNs. We use this branch to process downstream vision-audio-language tasks.
% \end{itemize}

% Although we use different adapters to encode the input of each modality, it may be difficult to accurately extract the information of these modalities using a naive Transformer architecture.
% Inspire by VLMO~\cite{vlmo} and BEIT-3~\cite{beit3}, we introduce three modality-specific FFNs in each Transformer block, the separate FFNs including Vision-FFN, Audio-FFN and Language-FFN.
% To encourage the interaction between different modalities, we also set a shared self-attention layer in each Transformer block.

% To encourage the interaction between different modalities, we set a shared self-attention layer in each Transformer block.

% To this end, we introduce three modality-specific to process the corresponding modalities, these FFNs including Vision FFN, Audio FFN and Language FFN.
% Also, 

% Inspire by VLMO~\cite{vlmo} and BEIT-3~\cite{beit3}, we introducd three modality-specific FFNs including Vision FFN, Audio FFN and Language FFN, to process the corresponding modalities. In addition, the self-attention  Different from xxx Unfortunately, we did not introduce modal interaction FFN (such as Vision-Language FFN, Audio-Language FFN) in the model. Using the Multiway Transformer structure can allow the model to perform various downstream tasks in different forms, for example, with the help of Vision FFN Perform vision tasks, perform Vision-Lanague tasks with Vision FFN and Language FFN, perform Audio-Lanague tasks with Audio FFN and Language FFN, and more. As shown in Figure xxx, 

\paragraph{Sub-LayerNorm} 
We introduce Sub-LayerNorm~\cite{magneto} to each Transformer block to increase training stability. 
Specifically, We insert layer normalization before the input projection and output projection of each self-attention layer and FFN layer. 
In our preliminary experiments, we find that Sub-LayerNorm can achieve better performance compared to the Pre-LayerNorm~\cite{gpt3}.
% Note that we did not use the initialization method of~\cite{magneto}, we find the model can train stably without the Magneto initialization.~\footnote{We train the model with Bfloat16 precision.}

\paragraph{GeGLU Activation Function} 
To further improve performance, we replace the activation function in FFN with GeGLU~\cite{glu} activation function. 
The intermediate dimension of FFN is set to $4$ times of the embedding dimension, which is consistent with the practice of PaLM~\cite{palm}.

\paragraph{Relative Position Bias (RPB)}
For positional information, we introduce 1D relative position bias~\cite{T5} for text and audio, and 2D relative position bias for image~\cite{coatnet}. 
At the pre-training stage, the relative position bias of different self-attention layers is shared. 
At the fine-tuning stage, we decouple the relative position bias of each self-attention layer and let them inherit the weights of the pretrained relative bias.

\paragraph{LayerScale} 
We introduce LayerScale~\cite{cait} to dynamically adjust the value of each residual block. Specifically, we multiply the output of each layer (e.g., self-attention layer and FFN) by a learnable diagonal matrix, whose values will be initialized to $1e-6$. In our preliminary experiments, LayerScale is beneficial for stabilizing training and improving performance.

\begin{figure*}[t]
\vskip 0.2in
    \centering
    \includegraphics[width=1\linewidth]{pic/pretraining_tasks.pdf}
    \caption{\textbf{The pretraining tasks of \onepeace.} Mask contrastive learning encourages the masked features close to the positive features (indicated by the green lines) and get away from the negative features (indicated by the red lines). Note that we compute the cross-modal contrastive loss by gathering features from all GPU devices, while the mask contrastive loss is computed on the local batch.}
    \label{fig:loss}
\end{figure*}

\subsection{Pretraining Tasks}
In this section, we present the pretraining tasks employed in \onepeace, including cross-modal contrastive learning and mask intra-modal contrastive learning. 
Cross-modal contrastive learning endows the model with cross-modal retrieval capability, while mask intra-modal contrastive learning enables the model to achieve superior fine-tuning performance on downstream tasks. 
An illustration of the pretraining tasks is shown in Figure~\ref{fig:loss}.
% Contrastive learning endows the model with powerful zero-shot retrieval capabilities. However, since contrastive learning pays more attention to the global representation of the samples, it tends to make the model ignore the internal details inside each sample.
% Recent works~\cite{beit3,fd-clip,EVA} have shown that using the features extracted by CLIP as the target for MIM Pretarining can improve the transfer effect of the student models on various vision or vision-language downstream tasks.
% Inspired by these works, we combine contrastive learning with Masked Modeling, allowing the model to learn both tasks simultaneously. It is hoped that the model can achieve good results after being migrated to downstream tasks of various modalities while maintaining good zero-shot retrieval capabilities.
% In particular, we found that simply using l1-loss or l2-loss for Masked Modeling will affect the effect of contrastive learning, so we modeled Masked Modeling as a Masked Contrastive Learning task, and we found that masked contrastive learning can be with contrastive learning compatible.

\subsubsection{Cross-Modal Contrastive Learning}
We perform cross-modal contrastive learning to align the semantic space of vision, language, and audio.
It contains both vision-language contrastive learning and audio-language contrastive learning.
Given an image-text pair $\left(I, T\right)$, we use the V-Branch and L-Branch to extract the image features and text features, respectively.
We regard the final output of vision class token and language class token as the global representations.
Followed by a linear projection and normalization, we obtain the image embedding $\bm{s}^V$ and language embedding $\bm{s}^L$.
Similarly, given an audio-text pair $\left( A, T'\right)$, we use the A-Branch and L-Branch to obtain the audio embedding $\bm{s}^A$ and language embedding $\bm{s}^{L'}$.
The contrastive loss functions are shown below:

\begin{equation}
\mathcal{L}_{CL-VL} = -\frac{1}{2N}\sum_{i=1}^{N}({\rm log}\frac{{\rm exp}(\bm{s}_i^{V}\bm{s}_i^{L}/\sigma)}{\sum_{j=1}^{N}{\rm exp}(\bm{s}_i^V\bm{s}_j^L/\sigma)} + {\rm log}\frac{{\rm exp}(\bm{s}_i^{V}\bm{s}_i^{L}/\sigma)}{\sum_{j=1}^{N}{\rm exp}(\bm{s}_j^V\bm{s}_i^L/\sigma)}),
\end{equation}

\begin{equation}
\mathcal{L}_{CL-AL} = -\frac{1}{2N}\sum_{i=1}^{N}({\rm log}\frac{{\rm exp}(\bm{s}_i^A\bm{s}_i^{L'}/\sigma)}{\sum_{j=1}^{N}{\rm exp}(\bm{s}_i^A\bm{s}_j^{L'}/\sigma)} + {\rm log}\frac{{\rm exp}(\bm{s}_i^A\bm{s}_i^{L'}/\sigma)}{\sum_{j=1}^{N}{\rm exp}(\bm{s}_j^A\bm{s}_i^{L'}/\sigma)}),
\end{equation}

where $\mathcal{L}_{VL}$ and $\mathcal{L}_{AL}$ refer to the vision-language contrastive loss and audio-language contrastive loss, respectively. $N$ is the batch size, $i,j$ are indexes within the batch, and $\sigma$ is a learnable temperature parameter (initialized to $0.07$).

% \paragraph{Audio-Language Contrastive Learning}
% Similaly, given an audio-text pair $\left( A, T\right)$, we denote the audio embedding as $h^A$, the audio-language contrastive loss function is shown below: 
% we denote the audio embedding as $h^A$, the audio-language contrastive loss function is shown below:

\subsubsection{Mask Intra-Modal Contrastive Learning}
% Inter-modal contrastive learning endows the model with powerful zero-shot retrieval capabilities. However, since inter-modal contrastive learning pays more attention to the global representation of the samples, it tends to make the model ignore the internal details inside each sample. 

% We strive to maintain the cross-modal retrieval capability of our model while achieving excellent performance when transferred to downstream tasks. 
% Initially, we considered combining cross-modal contrastive learning with the masked prediction task~\cite{bert,beit,mae}. 
% However, we found that directly integrating the masked prediction task would compromise the model's cross-modal retrieval ability. 
% To address this issue, we formulated the masked prediction task as a masked intra-modality contrastive learning task. 
% Our experiments indicate that masked intra-modality contrastive learning is highly compatible with cross-modal contrastive learning. 
% We subsequently apply mask intra-modality contrastive learning to each modality.

Cross-modal contrastive learning mainly focuses on aligning features between different modalities. 
However, it lacks emphasis on the learning of fine-grained details within modalities, leading to suboptimal finetuning performance in  downstream tasks~\cite{fd-clip}. 
To address this issue, we introduce mask intra-modal contrastive learning~\footnote{Mask intra-modal contrastive learning is similar to \cite{conmim}, but we extend it to more modalities.}.
It's still a form of contrastive learning, but unlike cross-modal contrastive learning, mask intra-modal contrastive learning focuses more on learning the fine-grained details within the modality.
Our experiment results show that it complements cross-modal contrastive learning and enhances the model's fine-tuning performance in downstream tasks. 
Next, we introduce how to apply mask intra-modal contrastive learning to various modalities.

\paragraph{Mask Vision Contrastive Learning}
Given an image, we randomly mask $75\%$ patches. Following~\cite{mae}, we only input the unmasked patches to the V-Branch to reduce computation costs and save memory. 
Then the encoded unmasked patches are concatenated with the mask token and fed to a lightweight Transformer decoder, which generates the corrupted features. 
In addition, the original image is fed to the vision branch to get the target features.
The corrupted features are learning to match the target features, the loss function is shown below:

\begin{equation}
\label{eq:mcl_v}
\mathcal{L}_{MCL-V} = -\frac{1}{N\hat{N}_V}\sum_{i=1}^{N}\sum_{j=1}^{\hat{N}_V}{\rm log}\frac{{\rm exp}(\bm{\hat{h}}_{ij}^V \cdot {\rm sg}(\bm{h}_{ij}^V)/\tau)}{\sum_{m=1}^{N}\sum_{n=1}^{N_V}{\rm exp}(\bm{\hat{h}}_{ij}^V  \cdot {\rm sg}(\bm{h}_{mn}^V)/\tau)},
\end{equation}

Where $\bm{\hat{h}}_{ij}^V$ denotes the representation of the masked patch, $\bm{h}_{ij}^V$ denotes the representation of the target patch, $\text{sg}(\cdot)$ denotes the stop gradient operation. $N$ is the batch size, $\hat{N}_V$ is the number of masked patches within a sample, $N_V$ is the number of whole patches within a sample. $\tau$ is a constant temperature value, we set it to $0.4$. 
This loss function not only encourages the masked patches close to the positive patches but also gets away from the negative patches.
As a result, each patch acquires a unique semantic meaning, which makes the model better transfer to downstream tasks.~\cite{fd-clip}

\paragraph{Mask Audio Contrastive Learning}
Given an audio, we sample $p=0.11$ of all time-steps to be starting indices and mask the subsequent $5$ time-steps. We manually adjust the mask rate to make approximately $55\%$ of all time steps to be masked for each sample. 
Similar to the image, the corrupted audio is encoded to the corrupted features, and the original audio is encoded to the target features.
The loss function is similar to Eq. (\ref{eq:mcl_v}), denoted as $\mathcal{L}_{MCL-A}$.

% \begin{equation}
% \label{eq:mcl_a}
% \mathcal{L}_{MCL-A} = -\frac{1}{N\hat{N}_A}\sum_{i=1}^{N}\sum_{j=1}^{\hat{N}_{A}}{\rm log}\frac{{\rm exp}(\bm{\hat{h}}_{ij}^A \cdot {\rm sg}(\bm{h}_{ij}^A)/\tau)}{\sum_{m=1}^{N}\sum_{n=1}^{N_A}{\rm exp}(\bm{\hat{h}}_{ij}^A \cdot {\rm sg}(\bm{h}_{mn}^A)/\tau)},
% \end{equation}

\paragraph{Mask Language Contrastive Learning}
Given a text, we randomly mask $15\%$ tokens of a text sequence. 
Different from BERT~\cite{bert}, we don't replace the masked token with the original tokens or random tokens. Instead, we only feed the unmasked tokens to the L-Branch, and get the final corrupted features through the Transformer decoder. 
The loss function is denoted as $\mathcal{L}_{MCL-L}$.
% The loss function of the mask language contrastive learning is shown below:

% \begin{equation}
% \label{eq:mcl_l}
% \mathcal{L}_{MCL-L} = -\frac{1}{N\hat{N}_L}\sum_{i=1}^{N}\sum_{j=1}^{\hat{N}_L}{\rm log}\frac{{\rm exp}(\bm{\hat{h}}_{ij}^L \cdot {\rm sg}(\bm{h}_{ij}^L)/\tau)}{\sum_{m=1}^{N}\sum_{n=1}^{N_L}{\rm exp}(\bm{\hat{h}}_{ij}^L \cdot {\rm sg}(\bm{h}_{mn}^L)/\tau)},
% \end{equation}

\paragraph{Mask Vision-Language Contrastive Learning}
Given an image-text pair, We randomly mask $68.75\%$ patches of the image and $40\%$ tokens of the text. 
We concatenate the unmasked patches and unmasked tokens, and encode them into the corrupted vision-language features through the VL-Branch and the Transformer decoders.
We also concatenate the original image patches and tokens, and encode them into the target vision-language features.
We use Equation~\ref{eq:mcl_v} to calculate the contrastive loss between the masked patch and the target patch, and Equation~\ref{eq:mcl_l} to calculate the contrastive loss between the masked token and the target token.
The average of these two losses forms the mask vision-language contrastive loss, denoted as $\mathcal{L}_{MCL-VL}$.

% \begin{align}
% \mathcal{L}_{MCL-VL-V} &= -\frac{1}{NN'_I}\sum_{i=1}^{N}\sum_{j=1}^{N'_I}{\rm log}\frac{{\rm exp}(\hat{h}_{ij}^Ih_{ij}^I/\tau)}{\sum_{m=1}^{N}\sum_{n=1}^{N_I}{\rm exp}(\hat{h}_{ij}^Ih_{mn}^I/\tau)} \notag \\
% \mathcal{L}_{MCL-VL-L} &= -\frac{1}{NN'_T}\sum_{i=1}^{N}\sum_{j=1}^{N'_T}{\rm log}\frac{{\rm exp}(\hat{h}_{ij}^Th_{ij}^T/\tau)}{\sum_{m=1}^{N}\sum_{n=1}^{N_T}{\rm exp}(\hat{h}_{ij}^Th_{mn}^T/\tau)} \notag \\
% \mathcal{L}_{MCL-VL} &= (\mathcal{L}_{MCL-VL-V} + \mathcal{L}_{MCL-VL-L})\ /\ 2
% \end{align}


\paragraph{Mask Audio-Language Contrastive Learning}
Given an audio-text pair, we randomly mask $45\%$ time-steps of the audio waveform and $40\%$ tokens of the text.
After going through a process similar to mask vision-language contrastive learning, we obtain corresponding corrupted features and target features. 
We denote the loss function of mask audio-language contrastive learning as $\mathcal{L}_{MCL-AL}$.

\subsection{Two-stage Pretraining}
\label{sec:two_stage_pretraining}
We divide the pretraining of \onepeace into two stages: vision-language pretraining and audio-language pretraining.
During the vision-language pretraining stage, the model only trains on image-text pairs and updates parameters that are relevant to vision and language.
The loss function at this stage is shown below:

\begin{equation}
\mathcal{L}_{VL} = \mathcal{L}_{CL-VL} + 1.0*\mathcal{L}_{MCL-V} + 0.5*\mathcal{L}_{MCL-L} + 1.0*\mathcal{L}_{MCL-VL}
\end{equation}

During the audio-language pretraining stage, the model trains solely on audio-text pairs, and we only update A-Adapter, A-FFNs, and other audio-related parameters. 
The remaining parameters including self-attention layers are totally frozen.
Despite not training on image-audio pairs, the semantic space between vision and audio is still aligned by using language as the anchor.
The loss function at the audio-language pretraining stage is shown below:

\begin{equation}
\mathcal{L}_{AL} = \mathcal{L}_{CL-AL} + 1.0*\mathcal{L}_{MCL-A} + 1.0*\mathcal{L}_{MCL-AL}
\end{equation}


% We denote a masked audio waveform representation, as 
% The loss function is shown below:
% \begin{align}
% \mathcal{L}_{MCL-AL-A} &= -\frac{1}{NN'_A}\sum_{i=1}^{N}\sum_{j=1}^{N'_A}{\rm log}\frac{{\rm exp}(\hat{h}_{ij}^Ah_{ij}^A/\tau)}{\sum_{m=1}^{N}\sum_{n=1}^{N_A}{\rm exp}(\hat{h}_{ij}^Ah_{mn}^A/\tau)} \notag \\
% \mathcal{L}_{MCL-AL-L} &= -\frac{1}{NN'_T}\sum_{i=1}^{N}\sum_{j=1}^{N'_T}{\rm log}\frac{{\rm exp}(\hat{h}_{ij}^Th_{ij}^T/\tau)}{\sum_{m=1}^{N}\sum_{n=1}^{N_T}{\rm exp}(\hat{h}_{ij}^Th_{mn}^T/\tau)} \notag \\
% \mathcal{L}_{MCL-AL} &= (\mathcal{L}_{MCL-AL-A} + \mathcal{L}_{MCL-AL-L})\ /\ 2
% \end{align}

\subsection{Pretraining Details}

\paragraph{Pretraining Datasets}
Our pretraining datasets are divided into two parts: image-text pairs and audio-text pairs. 
For image-text pairs, we use LAION-2B, a dataset obtained by web crawling.
For audio-text pairs, we collect a large amount of open-source environmental sound datasets.
For replication, all pretraining datasets are publicly available.
We provide more details about the pretraining datasets in Appendix~\ref{app:audio_text_data_details}.

% \paragraph{Pretraining Datasets}
% Our pretraining datasets are divided into two parts: image-text pairs and audio-text pairs. 
% For image-text pairs, we use LAION-2B, a pre-training dataset obtained by web crawling that may contain some noisy pairs. To improve the data quality, we apply several pre-processing steps, including removing images with an aspect ratio greater than 3.5, removing images with the shortest side less than 128, and removing images with a clip score less than 0.3. We also remove texts containing non-English or emoji characters, as well as texts with lengths less than 3 or greater than 512. After these steps, we retain about 1.5 billion image-text pairs.

% For audio-text pairs, we collect a large amount of open-source environmental sound datasets and perform simple cleaning on the data, which involves removing samples with text lengths less than 3 or greater than 512, as well as texts containing non-English or emoji characters. Ultimately, we preserve about 2.4 million audio-text pairs, with a total duration of around 8,000 hours. More information about the environmental sound data can be found in Appendix~\ref{app:audio_text_data_details}

\paragraph{Pretraining Settings}
\input{table/model_size}
\input{table/imagenet_result}
\onepeace is a giant-size model with $4$B parameters. We list the detailed hyper-parameters of \onepeace in Table~\ref{tb:model_configuration}. 
In addition, we introduce a lightweight Transformer decoder to recover the masked units from the visible units. The decoder is similar to the modality-fusion encoder, each block of it also consists of a shared self-attention layer and three modality-specific FFNs.
It has $2$ layers with $768$ hidden size, $2048$ intermediate size, and 12 attention heads.
The model weights of \onepeace are randomly initialized at the beginning, except for the feature extractor of A-adapter, for which we use the weights of WavLM~\cite{wavlm} for initialization. We find that a randomly initialized feature extractor can lead to overfitting, whereas incorporating the weights from WavLM significantly mitigated this problem and improve the performance.
More details about the pretraining settings are provided in Appendix~\ref{app:pretraining_hyperparameters}.

% As mentioned above, the pretraining of \onepeace is divided into two stages: vision-language pre-training and audio-language pretraining.
% For vision-language pretraining, we pretrain \onepeace for 200k steps with a batch size of 32768. We use the AdamW~\cite{adamw} optimizer with $(\beta_1,\beta_2)=(0.9, 0.98)$ and $\epsilon=1e\text{-}8$. The peak learning rate is set to $5e-4$, with a linear warmup of $3000$ steps and a cosine decay scheduler. The image resolution is set to $256\times256$. For regulation, we use weight decay with $0.05$ and disable dropout. We employ stochastic depth~\cite{drop-path} with a $0.4$ rate.
% For audio-language pretraining, we pretrain \onepeace for $10$ epochs with a batch size of $3072$. The peak learning rate is set to $2e-4$, with a linear warmup of $1$ epoch and cosine decay scheduler. Other hyper-parameters remain the same as vision-language pre-training.
% The model weights of \onepeace are randomly initialized at the beginning, except for the feature extractor of audio-adapter, for which we use the weights of WavLM~\cite{wavlm} for initialization. We found that a randomly initialized feature extractor can lead to overfitting, whereas incorporating the weights from WavLM significantly mitigated this problem and improve the performance.

\paragraph{Training Acceleration}
We introduce several model acceleration and memory optimization techniques to train \onepeace. 
First, we use memory-efficient attention~\cite{memory_efficient_attn,flash_attn} implemented in the Xformers library~\footnote{\url{https://github.com/facebookresearch/xformers/tree/main/xformers}} to save memory usage and improve training speed.
Secondly, we use the gradient checkpointing~\cite{checkpointing} technique to save memory, which allows us to use a larger batch size to train the model. 
In addition, we replace the layer normalization with Fused LayerNorm implemented in the Flash Attention library~\footnote{\url{https://github.com/HazyResearch/flash-attention}} and use nvFuser~\footnote{\url{https://github.com/pytorch/tutorials/blob/main/intermediate_source/nvfuser_intro_tutorial.py}} to fuse the operations of dropout, LayerScale, stochastic depth, and residual summing, which can bring some additional speed improvements. 
To improve the stability of model training and avoid gradient overflow issues, we use Bfloat16 precision to train \onepeace.

==> table/downstream_task.tex <==
\begin{table*}[t]
\normaltablestyle{8pt}{1.2}
\begin{tabular}{y{96}|cccccc}
Config & MSCOCO & Flickr30K & RefCOCO/$+$/g & VQA & NLVR2 \\
\shline
Optimizer & \multicolumn{5}{c}{AdamW} \\
Optimizer momentum & \multicolumn{5}{c}{$\beta_1, \beta_2{=}0.9, 0.999$} \\
Weight decay & \multicolumn{5}{c}{0.05} \\
Gradient clip & \multicolumn{5}{c}{0.0} \\
Warmup ratio & \multicolumn{5}{c}{0.1} \\
Learning rate schedule & \multicolumn{5}{c}{cosine decay} \\
Numerical precision & \multicolumn{5}{c}{$\mathtt{bf16}$} \\
Peak learning rate & 8e-5 & 7e-5 & 1.5e-4 & 3e-4 & 1e-4 \\
Layer-wise lr decay & 0.9 & 0.9 & 0.9 & 0.85 & 0.9 \\
Batch size & 3072 & 3072 & 256 & 512 & 128 \\
Training epochs & 15 & 20 & 30 & 10 & 25 \\
Drop path & 0.5 & 0.4 & 0.4 & 0.5 & 0.4 \\
Image resolution & 432 & 432 & 384 & 768 & 256 \\
\end{tabular}
\caption{\textbf{Fine-tuning setting} for vision-language tasks}
\label{tb:vision_language_config}
\end{table*}

==> table/instance_segmenation.tex <==
\begin{table*}[t]
\centering
\normaltablestyle{6pt}{1.2}
\begin{tabular}{y{85}|cc|cc}
Method                                 & Enc. \#Params & Crop Size & mIoU$^{ss}$ & mIoU$^{ms}$ \\
\shline
RevCol-H~\cite{cai2022reversible}      & 2.16B    & 640$^2$   & 60.4        & 61.0 \\
FD-SwinV2-G~\cite{wei2022contrastive}  & 3.00B    & 896$^2$   & -           & 61.4 \\
ViT-Adapter~\cite{chen2022vitadapter}  & 571M     & 896$^2$   & 61.2        & 61.5 \\
EVA~\cite{eva}                         & 1.01B    & 896$^2$   & 61.5        & 62.3 \\
BEiT-3~\cite{beit3}                    & 1.01B    & 896$^2$   & 62.0        & 62.8 \\
InternImage~\cite{wang2022internimage} & 1.08B    & 896$^2$   & \textbf{62.5}        & 62.9 \\
\hline
\modelname                             & 1.52B    & 896$^2$   & 62.0  & \textbf{63.0}
\end{tabular}
\caption{\textbf{System-level comparisons of semantic segmentation with leading results on ADE20k.} mIoU$^{ss}$ means single-scale inference result while mIoU$^{ms}$ means multi-scale.}
\label{tb:ade20k}
\end{table*}
